A neural network walks into a lab: towards using deep nets as models for human behavior

What might sound like the beginning of a joke has become an attractive prospect for many cognitive scientists: the use of deep neural network models (DNNs) as models of human behavior in perceptual and cognitive tasks. Although DNNs have taken over machine learning, attempts to use them as models of human behavior are still in the early stages. Can they become a versatile model class in the cognitive scientist's toolbox? We first argue why DNNs have the potential to be interesting models of human behavior. We then discuss how that potential can be more fully realized. On the one hand, we argue that the cycle of training, testing, and revising DNNs needs to be revisited through the lens of the cognitive scientist's goals. Specifically, we argue that methods for assessing the goodness of fit between DNN models and human behavior have to date been impoverished. On the other hand, cognitive science might have to start using more complex tasks (including richer stimulus spaces), but doing so might be beneficial for DNN-independent reasons as well. Finally, we highlight avenues where traditional cognitive process models and DNNs may show productive synergy.

==> For arXiv/glossary_openquestions.tex <==
\section*{Outstanding questions}
% should be phrased as questions
\begin{itemize}

    % Intro
    \item \textbf{A future for task-based training for higher cognition?} Inductive biases like convolution and hierarchical processing that have been used in computer vision (partly) coincidentally led DNNs to develop solutions similar to brain solution in object recognition. Inductive biases like attention or graph neural networks \cite{battaglia2018relational, vaswani2017attention} promise to yield success in more 'higher' cognitive tasks that require compositionality and flexible mapping of inputs to internal models of the world. Will these 'new' inductive biases similarly lead to coincidentally human-like solutions?

    % Designing
    \item \textbf{How can individual differences be captured in DNN models?} In comparing DNNs with humans, it is common to consider average human performance or to pool human data. Humans, however, have individual differences, Following cognitive process models, a DNN that purports to be a good model of human behavior should provide an account of individual differences. What will a DNN account of human inter-individual variability look like?
    
    \item \textbf{What is the role for toy tasks in neural network modeling?} In this review, we have advocated for cognitive tasks of higher complexity, primarily to pose challenges to human observers similar to the ones that machines have struggled to solve. This does not mean that we see no role for simple tasks and accompanying simple models. A toy task can represent the essence of a broad class of more complex or more real-world tasks. Understanding human or neural network behavior in a toy task can give us insights that generalize far beyond those tasks. However, we believe that ``representing the essence" and generalization should not be taken for granted. Scaling a task up in complexity (number of objects, number of interactions amongst objects, size of the state space, demands from other tasks, etc.) might force the brain or a neural network to use fundamentally different algorithms. In a given domain, what are the limitations of toy tasks and would scaling up task complexity make sense?
    
%    \item \textbf{A future for connectionism?} A parallel discussion point concerns the role of shallow %networks.
%    We have described that DNNs are in some way scaled-up, extra powerful connectionist networks. Viewed differently, however, the latter might still have advantages. Severely limiting the number of layers might help with interpretability and developing new predictions. Circumventing end-to-end learning by handcrafting task-relevant features might allow the researchers to focus on the computation of primary interest. When end-to-end learning is particularly challenging, a connectionist solution can set a benchmark for DNNs. Can connectionist networks retain a unique niche in between cognitive process models and DNNs?
    
%  \item {    While DNNs dominate machine learning, an artificial neural network does not need to be deep to account for human data in psychophysical paradigms that use strictly controlled, low-dimensional stimuli instead of natural ones (Orhan and Ma, 2017, Stoianov and Zorzi, 2012). At a mechanistic level, the resulting networks can be understood more easily than DNNs. Do such tasks and such networks have a future as toy models and tasks or do these combine the the worst of both worlds (not being powerful enough and still very hard to interpret)?
    
    \item \textbf{How sensitive are the emergent DNN models to their biological detail?} Incorporating more biological detail into DNNs will most likely increase their ability to display human-like behavior and internal activations. However, how 'smooth' is this space of biological realism - i.e., will small, critical changes in biological realism yield drastically different solutions or can we hope to adequately approximate human behavior and neural data by networks with very rudimentary biological detail? 

    \item \textbf{How may an account of probabilistic representations look like in a DNN?} Perceptual psychology has taught us that the human brain seem to represent uncertainty or even full probability distributions (reviewed in \cite{ma_neural_2014})). Bayesian probabilistic programs naturally incorporate this information \cite{lake_human-level_2015}, and probabilistic representations also emerge in trained shallow networks \cite{orhan_efficient_2017}, but does this generalize to DNNs \cite{kendall_what_2017} and can different types of uncertainty be distinguished \cite{gal_dropout_2016}?
    
    % EVALUATING
    
    \item \textbf{What are the limits of behavioral tests to discern between different models?} How far do we get with behavioral testing alone to adjudicate between competing models? This is already an important problem for cognitive process models but even more so for DNNs, as they are typically highly overparametrized. To what extent can models show the same detailed behavior but use very different algorithms and neural activations?

    % INCREASING
    
    \item \textbf{Will fitting DNNs to human behavior directly yield more human-like models?} In reference to Section \ref{directly}, can we expect more human-like out-of-distribution generalization from training DNNs directly on (large-scale) human behavior instead of the task optimal behavior? 

    \item \textbf{What are the prospects for simultaneous fitting of a DNN to behavioral and neural data}. Task-optimized DNNs are routinely “opened up” to examine the similarity of their internal representations to those of biological neurons. The same post-hoc analysis can be applied to a DNN optimized to match human data. Going further, what are the prospects for simultaneous fitting of a DNN to behavioral and neural data \cite{turner_why_2016, mcclure2016representational, kietzmann_recurrence_2019}?

    % cognitive process models vs. dnns?
    \item \textbf{What would a fair comparison between cognitive process models and DNNs look like?} When assessing the quantitative fit to human behavioral data, how should we weigh model complexity, the amount of training data, or the amount of incorporated domain knowledge when comparing cognitive process models and DNNs? In addition, the direct comparison of cognitive process models and DNN models remains rife with philosophical tension, relating to differing notions about the meaning of understanding \cite{cichy_deep_2019}. 
    
    \item \textbf{Towards embodied DNNs?} If we take the title of this paper way more seriously than anyone should, it could serve as a reminder that embodied cognition is still an under-explored area both in cognitive science and AI. Several ongoing projects try to endow virtual DNN agents with bodies that have to navigate  environments \cite{beattie2016deepmind, savva2019habitat}. Physical whole-body motor control \cite{wolpert_principles_2011} is even harder as well as the eventual integration of multiple cognitive functions such as perception and planning with motor control, such as in playing sports \cite{kitano1997robocup}.

    
\end{itemize}
